Understanding Gradient Descent on Edge of Stability in Deep Learning

Deep learning experiments by Cohen et al. [2021] using deterministic Gradient Descent (GD) revealed an Edge of Stability (EoS) phase when learning rate (LR) and sharpness (i.e., the largest eigenvalue of Hessian) no longer behave as in traditional optimization. Sharpness stabilizes around $2/$LR and loss goes up and down across iterations, yet still with an overall downward trend. The current paper mathematically analyzes a new mechanism of implicit regularization in the EoS phase, whereby GD updates due to non-smooth loss landscape turn out to evolve along some deterministic flow on the manifold of minimum loss. This is in contrast to many previous results about implicit bias either relying on infinitesimal updates or noise in gradient. Formally, for any smooth function $L$ with certain regularity condition, this effect is demonstrated for (1) Normalized GD, i.e., GD with a varying LR $\eta_t =\frac{\eta}{\| \nabla L(x(t)) \|}$ and loss $L$; (2) GD with constant LR and loss $\sqrt{L- \min_x L(x)}$. Both provably enter the Edge of Stability, with the associated flow on the manifold minimizing $\lambda_{1}(\nabla^2 L)$. The above theoretical results have been corroborated by an experimental study.

==> Gtbehavior.tex <==


\BehaviorGt*

%(1 + \Omega(\frac{\sin^2(\theta_t) \cos(\theta_t)}{ G_t } ))


\begin{proof}
    Using the Normalized GD update, we have
    \begingroup
    \allowdisplaybreaks
    \begin{align}
        &\langle v_1(t), x_{\eta} (t+1) - \Phi( x_{\eta} (t) ) \rangle - \langle v_1(t), x_{\eta} (t) - \Phi( x_{\eta} (t) ) \rangle \nonumber\\& = -\eta \frac{ \langle v_1(t), \nabla L( x_{\eta} (t) ) \rangle }{ \norm{ \nabla L( x_{\eta} (t) ) }  } \nonumber\\&
       = - \eta  \frac{ \langle v_1(t),  \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \frac{1}{2}   \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]  \rangle }{ \norm{ \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \frac{1}{2} \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]  } } \nonumber\\&+ O( \frac{\fourthL \secondL^2}{\mineigen^3} \eta^3) \label{eq:Gt_step1} \\&
       = - \eta  \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \frac{1}{2} v_1(t)^{\top}  \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]  }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \frac{1}{2} P_{t, \Gamma} \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]  } } \nonumber\\&+ O(\frac{\fourthL \secondL^2}{\mineigen^3} \eta^3) \label{eq:Gt_step2} \\&
       = - \eta  \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } +  \mathrm{err} +  O(\frac{\fourthL \secondL^2}{\mineigen^3} \eta^3) \label{eq:Gt_step3}.
    \end{align}
    \endgroup

    The steps followed above are as follows:
    \begin{enumerate}
        \item In \cref{eq:Gt_step1}, we use taylor expansion to expand $\nabla L( x_{\eta} (t))$ around $\Phi(x_{\eta} (t))$, with an error of $O(\fourthL \norm{ x_{\eta} (t) - \Phi(x_{\eta} (t))}^3)$. Since by alignment condition~\cref{eq:condition_perturbed},we have $\norm{ \tilde{x}_{\eta} (t) } \le O(\lambda_1(t) \eta)$, we have $\norm{x_{\eta} (t) - \Phi(x_{\eta} (t))} \le O( \frac{\lambda_1(t)}{\lambda_M(t)}) $.  This adds an error of magnitude $O(\frac{\fourthL \secondL^2}{\mineigen^3} \eta^3)$ to the entire term.
        %, after using \cref{ass:eigengap}.
         
        \item In \cref{eq:Gt_step2}, we divide the vector $\nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \frac{1}{2} \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]  $ using its projection onto the subspace $S_1$ spanned by $v_1(t), \ldots, v_M(t)$  and the subspace $S_2$ spanned by the rest of the eigenvectors $v_{M+1}(t), \ldots, v_{D}(t)$. Since $\nabla^2 L (\Phi(x_{\eta} (t)))$ only projects onto the subspace $S_1$, $S_2$ can only get its component from $\partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]$, which is of norm $O(\thirdL \norm{x_{\eta} (t) - \Phi (x_{\eta} (t))}^2)$. Thus, we can only consider the vector in $S_1$, with an error vector $O(\thirdL \norm{x_{\eta} (t) - \Phi (x_{\eta} (t))}^2)$ orthogonal to $S_1$. Taking the norm of this vector, we get an additional error term of magnitude  $O(\eta^4)$.
        
        \item In the final step (\cref{eq:Gt_step3}), we only consider $\nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ]$, which gives out an error term $\mathrm{err}$.
    \end{enumerate}
    
    
    
    Now, we show that $\abs{\mathrm{err}} \le O(\eta^2 \theta_t)$.
    
    
    First of all, $\norm{ \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))] } \le O(\thirdL \norm{x_{\eta} (t) - \Phi (x_{\eta} (t))}^2) = O( \frac{\thirdL \secondL^2}{\mineigen^2} \eta^2)$. Suppose $P_{t, \Gamma}^{(2:M)}$ denotes the projection matrix onto the subspace spanned by $v_2(t), \ldots, v_M(t)$, then denoting by $\mathrm{res}^{(2:M)}$ the vector $P_{t, \Gamma}^{(2:M)} \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]$ and by $\mathrm{res}$ the element $v_1(t)^{\top} \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]$, we have
    \begin{align}
        &\abs{\mathrm{res}}, \norm{\mathrm{res}^{(2:M)}} \le O( \frac{\thirdL \secondL^2}{\mineigen^2} \eta^2) \label{eq:boundresresperp}.
    \end{align}
    
    Thus, 
    \begin{align}
        &-\frac{1}{\eta} \mathrm{err} + \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } \nonumber\\&= 
        \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + v_1(t)^{\top}  \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]  }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \frac{1}{2} P_{t, \Gamma} \partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]  } } \label{eq:Gt_step4}
        \\& = \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \mathrm{res} }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] +  \mathrm{res} \cdot v_1(t) + \mathrm{res}^{(2:M)} } } \label{eq:Gt_step5}\\&
        =  \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \mathrm{res} }{ \sqrt{ (v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \mathrm{res})^2 +  \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \mathrm{res}^{(2:M)} }^2 } } \label{eq:Gt_step6} \\&
        = \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } \left[ \sqrt{1 + \mathrm{err}' }\right] \nonumber%\label{eq:Gt_step7}%\\&
        %= (1 + \mathrm{err}') \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }, \label{eq:Gt_step8}.
    \end{align}
    where 
    $$
        \mathrm{err}' = \frac{ \left[ \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } \right]^2 - \left[ \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ]  +  \mathrm{res}^{(2:M)} } }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \mathrm{ res } } \right]^2 } {1 + \left[ \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } \right]^2 }.
    $$ 
    We followed the following steps in the above set of equations:
    \begin{enumerate}
        \item In \cref{eq:Gt_step4}, we just copied the term from \cref{eq:Gt_step2}, which was divided into terms $\mathrm{err}$ and $\frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }$.
        
        \item In \cref{eq:Gt_step5}, we introduced the terms $\mathrm{res}$ and $\mathrm{res}^{(2:M)}$ to represent $\partial^2 (\nabla L) (\Phi(x_{\eta} (t))) [x_{\eta} (t) - \Phi (x_{\eta} (t)), x_{\eta} (t) - \Phi (x_{\eta} (t))]$.
        
        \item In \cref{eq:Gt_step6}, we expanded the norm in the denominator using the projection along the vector $v_1(t)$ and the subspace spanned by $v_2(t), \ldots, v_M(t)$.
        %\item In \cref{eq:Gt_step7}, we used a simple modification to
        %\item
    \end{enumerate}
    
    
    
    The magnitude of $\mathrm{err}'$ can now be bounded as follows:
    \begingroup
    \allowdisplaybreaks
    \begin{align}
        &
        \abs{\mathrm{err}'} = \abs{ \frac{ \left[ \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } \right]^2 - \left[ \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ]  +  \mathrm{res}^{(2:M)} } }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \mathrm{ res } } \right]^2 } {1 + \left[ \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } \right]^2 } } \nonumber\\&
        = \frac{1}{\sec^2 \theta_t}\Big|  \left[ \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } \right]^2 \nonumber\\&- \left[ \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ]  +  \mathrm{res}^{(2:M)} } }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \mathrm{ res } } \right]^2  \Big| \label{eq:Gt_step8}\\&
        \le O\left(  \frac{1}{G_t \lambda_1(t) \sec^2 \theta_t} (\norm{\mathrm{res}^{(2:M)}} + \abs{\mathrm{res}} \tan \theta_t  )  \cdot \abs{ \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{ v_1^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } \right) \label{eq:Gt_step9}\\&
        %\le O\left( \frac{1}{G_t} (\norm{\mathrm{res}^{(2:M)}} + \abs{\mathrm{res}} )  \cdot \abs{ \frac{ \norm{ P_{t, \Gamma}^{(2:M)}  [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{v_1^{\top}  [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } \right) \\&
        \le O\left( \frac{1}{G_t \lambda_1(t)} (\norm{\mathrm{res}^{(2:M)}} + \abs{\mathrm{res}} \tan \theta_t  )  \cdot \abs{ \sin 2\theta_t } \right). \label{eq:Gt_step10}
    \end{align}
    \endgroup
    
     We followed the following steps in the above set of equations:
    \begin{enumerate}
        \item In \cref{eq:Gt_step8}, we used the definition of $\theta_t$ to represent $\frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{ v_1^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }.$ 
        
        
        \item In \cref{eq:Gt_step9}, we bound the magnitude of $\frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } + \mathrm{res} }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \mathrm{res}^{(2:M)} }$ by
        \begin{align*}
            &\abs{\frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } + \mathrm{res}^{(2:M)} }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] + \mathrm{res} }} \\&\le \abs{\frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }} \\& + O\Big( \frac{1}{\abs{ v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } \\& \cdot \Big(\norm{\mathrm{res}^{(2:M)}} + \abs{\mathrm{res}} \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{ \abs{ v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } \Big) \Big) \\&
            = \frac{ \norm{ P_{t, \Gamma}^{(2:M)} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }{ \abs{ v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }}  + O\left( \frac{1}{G_t \lambda_1(t)} \left(\norm{\mathrm{res}^{(2:M)}} + \abs{\mathrm{res}} \tan \theta_t \right) \right).
        \end{align*}
         In the final step, we have used the following steps:
        $$
        \abs{ v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } = \abs{ \lambda_1(t) v_1(t)^{\top} [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ]} = \lambda_1(t) G_t.
        $$
        The pre-final step is true iff $G_t > \Omega( \norm{\mathrm{res}^{(2:M)}} + \abs{\mathrm{res}} )$. Since we have a bound of $O(\frac{\thirdL \secondL^2}{\mineigen^2}  \eta^2)$ on $\abs{\mathrm{res}}, \norm{\mathrm{res}^{(2:M)}}$ from \cref{eq:boundresresperp}, having a lower bound of $\Omega(\eta^{1.5})$ on $G_t$ suffices, provided $\eta \le O( \frac{\mineigen^4}{\thirdL^2 \secondL^4}  )$.
        %\item In \cref{eq:Gt_step7}, we used a simple modification to
        %\item
    \end{enumerate}
    
    
    Hence, combining everything, we have
    \begin{align*}
        \abs{ \mathrm{err} } &\le \eta \abs{\sqrt{1 + \mathrm{err}'} - 1} \abs{\frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }} \\&
        \le \eta O(\abs{ err' }) \\&
        \le O (\frac{\thirdL \secondL^2 \eta^3}{\mineigen^2 G_t \lambda_1(t)} \sin \theta_t),
    \end{align*}
    where in the second step, we have used the fact that $\abs{\frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } }} = \abs{\cos \theta_t} < 1$.
    
    
    Thus, continuing from \cref{eq:Gt_step3}, we have
    \begin{align}\label{eq:noisyfirstcoordinateupate_Gt}
        \langle v_1(t), x_{\eta} (t+1) - \Phi( x_{\eta} (t) ) \rangle - \langle v_1(t), x_{\eta} (t) - \Phi( x_{\eta} (t) ) \rangle &= - \eta  \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } \nonumber \\&+ O( \frac{\fourthL \secondL^2}{\mineigen^3}  \eta^3 + \frac{\thirdL \secondL^2 \eta^3}{\mineigen^2 \lambda_1(t) G_t} \sin \theta_t ).
    \end{align}
    Similarily, we can show
    \begin{align*}
        &\langle v_1(t), x_{\eta} (t+2) - \Phi( x_{\eta} (t) ) \rangle - \langle v_1(t), x_{\eta} (t+1) - \Phi( x_{\eta} (t) ) \rangle \\&= - \eta  \frac{v_1(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t+1) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t+1) - \Phi ( x_{\eta} (t) ) ] } } \\&+ O\left( \frac{\fourthL \secondL^2}{\mineigen^3} \eta^3 + \frac{\thirdL \secondL^2\eta^3}{ \mineigen^2 \abs{ v_1(t)^{\top} \nabla^2 L ( \Phi ( x_{\eta} (t) ) ) [ x_{\eta} (t+1) - \Phi(x_{\eta} (t))] } } \sin \tilde{\theta}_t \right),
    \end{align*}
    where $\cos \tilde{\theta_t} = \frac{ \abs{ v_1(t)^{\top} \nabla^2 L ( \Phi ( x_{\eta} (t) ) ) [ x_{\eta} (t+1) - \Phi(x_{\eta} (t))] } }{ \norm{P_{t, \Gamma} \nabla^2 L ( \Phi ( x_{\eta} (t) ) ) [ x_{\eta} (t+1) - \Phi(x_{\eta} (t))] } }$. 
    Hence, we can combine the two equations to have
    \begin{align}
        \langle v_1(t), x_{\eta} (t+2) - \Phi( x_{\eta} (t) ) \rangle =  
         a_{t+1} a_{t} \langle v_1(t), x_{\eta} (t+2) - \Phi( x_{\eta} (t) ) \rangle + \overline{\mathrm{err}}, \label{eq:updateinGt}
    \end{align}
    where
    \begin{align*}
        a_{t+1} &= 1 - \frac{ \eta \lambda_1(t) }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t+1) - \Phi ( x_{\eta} (t) ) ] } },\\
        a_t &= 1 - \frac{ \eta \lambda_1(t) }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } ,\\
        \abs{ \overline{\mathrm{err}} } &\le \abs{a_{t+1}}O( \frac{\fourthL \secondL^2}{\mineigen^3}\eta^3 + \frac{\thirdL \secondL^2\eta^3}{ \mineigen^2 G_t \lambda_1(t)} \sin \theta_t ) \\&+ O\left( \frac{\fourthL \secondL^2}{\mineigen^3} \eta^3 + \frac{\thirdL \secondL^2 \eta^3}{ \mineigen^2 \abs{ v_1(t)^{\top} \nabla^2 L ( \Phi ( x_{\eta} (t) ) ) [ x_{\eta} (t+1) - \Phi(x_{\eta} (t))] } } \sin \tilde{\theta}_t \right).
    \end{align*}
    Using \cref{lem:behaviornormhalf_general} that predicts an increase (albeit an error of $O(\eta^2)$) on the projection along the top eigenvector, we have
    \begin{align*}
        \abs{ \overline{\mathrm{err}} } \le \abs{a_{t+1}}O( \frac{\fourthL \secondL^2}{\mineigen^3} \eta^3 + \frac{\thirdL \secondL^2 \eta^3}{\mineigen^2 G_t \lambda_1(t)} \sin \theta_t ) + O\left( \frac{\fourthL \secondL^2}{\mineigen^3} \eta^3 + \frac{\thirdL \secondL^2 \eta^3}{\mineigen^2 G_t \lambda_1(t)} \sin \theta_t \right).
    \end{align*}
    Since, 
    \begin{align*}
    \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t+1) - \Phi ( x_{\eta} (t) ) ] } &\ge  \abs{ v_1(t)^{\top}  \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t+1) - \Phi ( x_{\eta} (t) ) ] } \\&\ge \frac{1}{2}\abs{ v_1(t)^{\top}  \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } = \frac{1}{2} \lambda_1(t) G_t,
    \end{align*}
    using \cref{lem:behaviornormhalf_general}, that predicts an increase (albeit an error of $O(\eta^2)$) on the projection along the top eigenvector, in the pre-final step, we have $\abs{a_{t+1}} \le \frac{2 \eta}{G_t}$. Thus, overall,
    \begin{align*}
        \abs{ \overline{\mathrm{err}} } \le O\left( \frac{\fourthL \secondL^2 \eta^4}{\mineigen^3 G_t} + \frac{\thirdL \secondL^2 \eta^4}{\mineigen^2 G^2_t  \lambda_1(t)} \sin \theta_t + \frac{\fourthL \secondL^2 \secondL}{\mineigen^3} \eta^3 + \frac{\thirdL \secondL^2 \eta^3}{\mineigen^2 G_t \lambda_1(t)} \sin \theta_t \right).
    \end{align*}
    
    Using the steps used for finding the noisy quadratic update rule of Normalized GD in \cref{lem:appr_gradient_norm} ( \cref{eq:noisynormaliedgdupdate_primal} ), we can show that
    \begin{align}\label{eq:noisysecondcoordinateupate_Gt}
        &\langle v_j(t), x_{\eta} (t+1) - \Phi( x_{\eta} (t) ) \rangle - \langle v_j(t), x_{\eta} (t) - \Phi( x_{\eta} (t) ) \rangle \nonumber\\&= - \eta  \frac{v_j(t)^{\top} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }{ \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } } + O(\frac{\thirdL \secondL}{\mineigen}\eta^2),
    \end{align}
    for all $2 \le j \le M$. Hence, with \cref{eq:noisyfirstcoordinateupate_Gt} and \cref{eq:noisysecondcoordinateupate_Gt}, we can further show that 
    \begin{align}
        \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t+1) - \Phi ( x_{\eta} (t) ) ] } &\le  \eta \lambda_1(t) - \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } \nonumber\\&- 2 \eta \min_{2 \le j \le M} \frac{\lambda_j(t) ( \lambda_1(t) - \lambda_j(t) ) }{ \lambda_1(t) } \sin^2 \theta_t \\& + O( \frac{\thirdL \secondL}{\mineigen}\eta^2 \sin \theta_t + \frac{\fourthL \secondL^2}{\mineigen^3}  \eta^3 + \frac{\thirdL \secondL^2 \eta^3}{\mineigen^2 \lambda_1(t) G_t} \sin \theta_t ) \label{eq:updateinnorm_general}.
    \end{align}
    Further, from alignment condition(\cref{eq:condition_perturbed}), we have
    \begin{align*}
        \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t+1) - \Phi ( x_{\eta} (t) ) ] }&, \norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] } \\& \le \lambda_1 (t) \eta
        + O( \thirdL \secondPhi  \eta^2  ) + O(\frac{\thirdL \secondL^2 \secphaseinit}{\mineigen^2} \eta^2  ) \\&+  O( \sqrt{D} \secondPhi \secondL \secphaseinit \thirdL  \eta^2   ) + O(\eta^2 D) \\& \le 2\lambda_1(t) \eta,
    \end{align*}
    if $\eta \le O (\frac{\mineigen^3}{\thirdL \secondPhi \secphaseinit \secondL^2 D }) .$
    
    Continuing from \cref{eq:updateinGt}, we have
    \begin{align}
        \abs{ \langle v_1(t), x_{\eta} (t+2) - \Phi( x_{\eta} (t) ) \rangle } &=  
         \abs{ a_{t+1} a_{t} \langle v_1(t), x_{\eta} (t) - \Phi( x_{\eta} (t) ) \rangle } + \overline{\mathrm{err}} \nonumber\\&
        \ge ( 1 + \frac{1}{2} \min_{2 \le j \le M} \frac{\lambda_j(t) ( \lambda_1(t) - \lambda_j(t) ) }{ \lambda^2_1(t) } \sin^2 \theta_t ) G_t + \Tilde{\mathrm{err}}, \label{eq:G_tfinalbound}
    \end{align}
    where we use \cref{eq:updateinnorm_general} and the bounds on $\norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t+1) - \Phi ( x_{\eta} (t) ) ] }$, $\norm{ P_{t, \Gamma} \nabla^2 L (\Phi(x_{\eta} (t))) [ x_{\eta} (t) - \Phi ( x_{\eta} (t) ) ] }$ in the final step, with 
    \begin{align*}
        \abs{ \Tilde{\mathrm{err}} } &\le \overline{\mathrm{err}} + \frac{G_t}{2 \eta \lambda_1(t)} O( \frac{\thirdL \secondL}{\mineigen}\eta^2 \sin \theta_t + \frac{\fourthL \secondL^2}{\mineigen^3}  \eta^3 + \frac{\thirdL \secondL^2 \eta^3}{\mineigen^2 \lambda_1(t) G_t} \sin \theta_t )  \\&
        \le O( \frac{\fourthL \secondL^2}{\mineigen^3} \eta^3 + (1 + \eta / G_t) \frac{\thirdL \secondL^2\eta^3}{\mineigen^2 \lambda_1(t) G_t} \sin \theta_t ). 
    \end{align*}
    The proof now follows from \cref{eq:G_tfinalbound}, after taking into account $\norm{v_1(t) - v_1(t+2)}$ and $\norm{\Phi ( x_{\eta} (t+2) )  - \Phi ( x_{\eta} ( t ) }$. From \cref{lem:boundmovementinPhi}, we have $\norm{\Phi(x_{\eta} (t)) - \Phi(x_{\eta} (t+1))} \le O(\secondPhi \eta^2)$, which further implies, $\norm{ \nabla^2 L(\Phi(x_{\eta} (t+1))) - \nabla^2 L(\Phi(x_{\eta} (t))) } \le O( \thirdL \secondPhi \eta^2 ) $. Thus, we can use \cref{lem:DavisKahn} to have $\norm{v_1(t) - v_1(t+1)} \le O( \frac{\thirdL \secondPhi \eta^2 }{ \lambda_1(t) - \lambda_2(t) } ) = O( \frac{\thirdL \secondPhi \eta^2 }{ \eigengap } ) $. From \cref{lem:PhiGt}, we have $\abs{ \langle v_1(t), \Phi(x_{\eta} (t+1)) - \Phi(x_{\eta} (t)) \rangle} \le O( \frac{\secondPhi \secondL \thirdL \thirdPhi \eta^3}{\mineigen^2 } ).$ Thus,
    
    \begin{align*}
        G_{t+2} &= \abs{ \langle v_1(t+2), x_{\eta} (t+2) - \Phi( x_{\eta} (t+2) ) \rangle } \\&= \abs{ \langle v_1(t), x_{\eta} (t+2) - \Phi( x_{\eta} (t) ) \rangle } + O(  \frac{\thirdL \secondPhi \eta^3 }{ \eigengap } +  \frac{\secondPhi \secondL \thirdL \thirdPhi \eta^3}{\mineigen^2 \eigengap} ) \\&
       \ge ( 1 + \frac{1}{2} \min_{2 \le j \le M} \frac{\lambda_j(t) ( \lambda_1(t) + O(\normerrterm \eta) - \lambda_j(t) ) }{ \lambda^2_1(t) } \sin^2 \theta_t ) G_t \\& +  O( \frac{\fourthL \secondL^2}{\mineigen^3} \eta^3 + (1 + \eta / G_t) \frac{\thirdL \secondL^2\eta^3}{\mineigen^2 \lambda_1(t) G_t} \sin \theta_t ) + O(  \frac{\thirdL \secondPhi \eta^3 }{ \eigengap } +  \frac{\secondPhi \secondL \thirdL \thirdPhi \eta^3}{\mineigen^2 } ) \\&\ge ( 1 + \frac{1}{4} \min_{2 \le j \le M} \frac{\lambda_j(t) ( \lambda_1(t) + O(\normerrterm \eta) - \lambda_j(t) ) }{ \lambda^2_1(t) } \sin^2 \theta_t ) G_t \\& +  O( \frac{\fourthL \secondL^2}{\mineigen^3} \eta^3 + (1 + \eta / G_t) \frac{\thirdL \secondL^2\eta^3}{\mineigen^2 \lambda_1(t) G_t} \sin \theta_t ) + O(  \frac{\thirdL \secondPhi \eta^3 }{ \eigengap } +  \frac{\secondPhi \secondL \thirdL \thirdPhi \eta^3}{\mineigen^2 } ).
    \end{align*}
    The error term in the pre-final step can be further upper bounded as as $O( \frac{\fourthL \secondL^2 \secondPhi \thirdL \thirdPhi }{\mineigen^3 \Delta} \eta^3 + (1 + \eta / G_t) \frac{\thirdL \secondL^2\eta^3}{\mineigen^2 \lambda_1(t) G_t} \sin \theta_t ) $. The final step follows if $\eta \le O(\frac{\eigengap}{\normerrterm})$.
    %\todo{Lol! need to show the movement along top eigenvector is eta3 }
    
    %The above equation will follow from using the same proof used in \cref{lemnma}
    
    %Thus, the Normalized GD update is equivalent to the update in the quadratic model with an error of $O( \fourthL \eta^3 + \frac{\thirdL \eta^3}{G_t} sin \theta_t )$ and hence, the rest of the proof will follow from using similar technique as in lemma~\ref{lem:firscoordincr_ondrop}.
    
    
    
    
\end{proof}

